Uncovering Weaknesses in Neural Code Generation

Code generation, the task of producing source code from prompts, has seen significant advancements with the advent of pre-trained large language models (PLMs). Despite these achievements, there lacks a comprehensive taxonomy of weaknesses about the benchmark and the generated code, which risks the community's focus on known issues at the cost of under-explored areas. Our systematic study aims to fill this gap by evaluating five state-of-the-art PLMs: three larger models, CodeGen2.5 with 7 billion parameters, CodeGeeX2 with 6 billion parameters, GPT-4 Turbo, and two smaller ones, UnixCoder with 110 million parameters and CodeT5 base with 220 million parameters, across three popular datasets, CoNaLa, HumanEval Plus, and DS-1000. We assess the quality of generated code using match-based and execution-based metrics, then conduct thematic analysis to develop a taxonomy of nine types of weaknesses. We dissected weakness distributions in both larger and smaller models, applying an extensive methodology that encompasses model-specific as well as collective analysis (union and intersection) across models. Our research uncovers three salient findings: 1. In the CoNaLa dataset, inaccurate prompts are a notable problem, causing all large models to fail in 26.84% of cases, with even higher failure rates of 40% for smaller models; 2. Missing pivotal semantics is a pervasive issue across benchmarks, with one or more large models omitting key semantics in 65.78% of CoNaLa tasks, and similarly high occurrences in HumanEval Plus (66.09%) and DS-1000 (80.51%); 3. All models struggle with proper API usage, a challenge amplified by vague or complex prompts. Our findings aim to steer researchers towards addressing specific weaknesses and challenges in code generation. Furthermore, our annotations can offer a targeted benchmark subset for detailed analysis.

==> sections/Background.tex <==
\section{Background}
\label{sec:background}

==> sections/Hypothesis.tex <==
\section{Two preliminary studies}
\label{sec:preliminaryStudy}
% test
\setParDisTest
We are interested in exploring the efficacy of addressing the identified weaknesses in prompts for code generation, and whether the weaknesses identified from medium-scale code-PLMs persist in SOTA commercial LLM ChatGPT. Thus, we conducted two preliminary studies to answer the following two research questions (RQs).\\
\noindent \emph{RQ1: Can the quality of generated code be significantly improved by addressing the identified weaknesses in prompts? }\\
\noindent \emph{RQ2: Can the identified prompt- and model-related weaknesses be applied to ChatGPT?}\\


\noindent \textbf{RQ1: Significance of addressing weaknesses in prompts.} In Section \ref{subsec:promptWeakness}, we highlighted three types of prompt weaknesses. We hypothesize that rectifying these issues may potentially enhance the quality of generated code. To evaluate it, we conducted a preliminary study by randomly selecting prompts, modifying them, re-running the models to generate code, and comparing the quality of generated code based on original and modified prompts. In addition to the four models previously discussed, we also assess the influence of prompts on ChatGPT, given its outstanding performance in code generation.

 To maintain fairness, the selection of cases was performed exclusively from the test dataset, ensuring that neither of the models had any exposure to the prompts during their training or fine-tuning phase. From Table \ref{tab:weaknessDistribution}, the number of samples exhibiting `too complex' weaknesses in CoNaLa, as well as those showing `lack of domain knowledge' weaknesses in both CoNaLa and HumanEval, is 15. While considering the sample size and our modification effort, we set 15 as our threshold. For weakness types with a case count exceeding 15, we randomly selected 15 cases from that particular set. In cases where the number of cases for a weakness type was less than 15, we included all available cases without any random selection. The numbers of cases across the three datasets are shown in Table \ref{tab:randomSample}.


%%%%%%%%%%for limited space
\begin{table}[!htbp]
        \centering
        \footnotesize
        %\scriptsize
        \caption{Counts of Chosen Cases by Weakness Type}
        \label{tab:randomSample}
        \begin{tabular}{|p{2cm}|c|c|c|c|}
        \hline
        \multicolumn{2}{|c|}{\textbf{Weaknesses}} & \textbf{CoNaLa} & \textbf{HumanEval} & \textbf{DS-1000} \\ \hline
        \multirow{3}{*}{Inaccurate desc.} & Vagueness & 15 & 1 & 0 \\ \cline{2-5}
        & Incompleteness & 15 & 0 & 0 \\ \cline{2-5}
        & Inconsistency & 15 & 0 & 0 \\ \hline
        \multicolumn{2}{|c|}{Too complex prompts} & 15 & 7 & 15 \\ \hline
        \multicolumn{2}{|c|}{Grammar errors} & 5 & 0 & 0 \\ \hline
        \end{tabular}
\end{table}

Several outstanding resources provide guidelines for writing effective prompts, including the online course by Andrew Ng and Isa Fulford \cite{onlineCourse}, as well as explorative studies on reusable prompt patterns \cite{white2023prompt, mishra-etal-2022-reframing}.  Although the adjustments vary based on different types of weakness, the overarching objective remains consistent: to enhance the clarity and specificity of the prompts. Our primary strategies include clarifying the target, filtering potential distracting statements (e.g., invalid attempts and source code for a problem), furnishing essential details, breaking down complex tasks into simpler sequential steps, and imparting vital background information. For example, when a prompt requires counting vowels, we provide a definition of what constitutes a vowel. 

An example for each distinct type of weakness has been included for clarity, while all other revised prompts can be accessed through the provided artifact URL. However, our rectification process does not necessarily represent an exemplar for crafting optimal prompts; it represents merely a preliminary exploration.

%test
\setParDefTest
\setParDis

\noindent \textbf{I.i. Vagueness:} For vague prompts, we initially enhance clarity by supplying more specific information or examples, altering ambiguous words or phrases, and defining terms that may have multiple meanings. Just as in the following example, we give more detailed explanation about the sum calculation of ``nested list''.

   \begin{PromptCode}[language=Python]
Initial prompt:sum all elements of nested list `L`
Answer: sum(sum(i) if isinstance(i, list) else i for i in L)
\end{PromptCode}
\vspace{-11pt}

\begin{T5Code}[language=Python]
Rewritten prompt: sum all elements of nested list 'L', and if an element is a 
list, compute its sum before adding it to the final result.
\end{T5Code}
\vspace{-10pt}

 \noindent \textbf{I.ii. Incompleteness:} Our observations indicate that incomplete semantic weaknesses primarily stem from missing parameters, storage format, special operations, etc., in the prompts, as compared to the reference source code. Consequently, for prompts exhibiting this type of weakness, we simply supplement the missing information, as illustrated in the following example.

  \begin{PromptCode}[language=Python]
Initial prompt:create a random list of integers
Answer: [int(1000 * random.random()) for i in range(10000)]
\end{PromptCode}
\vspace{-12pt}

\begin{T5Code}[language=Python]
Rewritten prompt:create a random list of 10000 integers between 0 and 999.
\end{T5Code}
\vspace{-10pt}

\noindent \textbf{I.iii. Inconsistency:} This type of weakness is rectified by modifying the prompt to accurately reflect the intention of the reference source code. In the following example, we eliminate the negative instance to ensure consistency between the prompt and the reference source code.
 \begin{PromptCode}[language=Python]
Prompt:def sort_array(arr):
"""
In this Kata, you have to sort an array of non-negative integers according to 
number of ones in their binary representation in ascending order. For similar 
number of ones, sort based on decimal value. It must be implemented like this:
>>> sort_array([1, 5, 2, 3, 4]) == [1, 2, 3, 4, 5]
>>> sort_array([-2, -3, -4, -5, -6]) == [-6, -5, -4, -3, -2]
>>> sort_array([1, 0, 2, 3, 4]) == [0, 1, 2, 3, 4]
"""
Answer: return sorted(sorted(arr), key=lambda x: bin(x)[2:].count('1'))
\end{PromptCode}
\vspace{-15pt}

\begin{T5Code}[language=Python]
Rewritten prompt: def sort_array(arr):
"""
In this Kata, you have to sort an array of non-negative integers according to 
number of ones in their binary representation in ascending order. For similar
number of ones, sort based on decimal value. It must be implemented like this:
>>> sort_array([1, 5, 2, 3, 4]) == [1, 2, 3, 4, 5]
>>> sort_array([1, 0, 2, 3, 4]) == [0, 1, 2, 3, 4]
"""
\end{T5Code}
\vspace{-10pt}

\noindent \textbf{II. Too complex prompts:} Most of the cases involving intertwined steps or lack of necessary knowledge. Thus, we disentangle and organize them as itemizing instructions, just as the illustration in the following example. If the prompts are overly lengthy with numerous subordinate clauses and prepositional phrases, we convert these long sentences into multiple shorter ones, curtailing the use of clauses.

 \begin{PromptCode}[language=Python]
Prompt:def sort_third(l: list):
"""
This function takes a list l and returns a list l' such that l' is identical to 
l in the indicies that are not divisible by three, while its values at the 
indicies that are divisible by three are equal to the values of the 
corresponding indicies of l, but sorted.
>>> sort_third([1, 2, 3])
[1, 2, 3]
>>> sort_third([5, 6, 3, 4, 8, 9, 2])
[2, 6, 3, 4, 8, 9, 5]
"""
Answer: 
    l = list(l)
    l[::3] = sorted(l[::3])
    return l
\end{PromptCode}
\vspace{-15pt}

\begin{T5Code}[language=Python]
Rewritten prompt: This function takes a list l and returns a new list l'. The 
assignment rules for l' are as follows:
1. In l', all elements at indices not divisible by three are identical to those
in the original list l.
2. For all elements at indices that are multiples of three, they are derived 
from corresponding elements in the original list l, arranged in ascending order,
and placed sequentially.
\end{T5Code}
\vspace{-12pt}

For prompts exhibiting grammatical errors, we simply rectify them. We will not present examples here. Once we compiled all revised prompts, we retested them on the four models being evaluated. Specifically, for CoNaLa samples, we retested them on the four fine-tuned models. Meanwhile, HumanEval and DS-1000 samples were tested on the fine-tuned CodeT5-based and UnixCoder, and directly on the two larger models. For the prompts with multiple weaknesses, the version fixing only one certain weakness is used for comparison. Given the inherent randomness of PLMs, we conducted ten iterations for each model on every prompt, including both the original and our rewritten versions, from which we computed the average score. In pursuit of demonstrating the significance of prompt clarification, we calculated the difference in average scores (i.e., $score_{rewritten} - score_{ori.}$ ), and present these results in Table \ref{tab:rewrittenPrompt}. 

%test
\setParDef
\setParDisTest

In summary, the clarification of prompts appears to broadly enhance the quality of the code generated by the five models under study – this improvement is evidenced by 34 wins out of 40 comparisons. Importantly, all five models showed superior performance with prompts that effectively addressed issues including vagueness, complex statements, and grammatical errors in CoNaLa. Notably, the largest model, ChatGPT, demonstrated consistent excellence across all rewritten prompts from all three datasets on average.

However, it's worth noting that even after adopting the latest best practices \cite{onlineCourse, white2023prompt, mishra-etal-2022-reframing} for prompt rewriting, some models (including ChatGPT) displayed inferior performance for certain prompts. This underscores the understanding that improved prompts do not universally guarantee enhanced performance for code-PLMs. While the quality of prompts can indeed influence the code generation quality, its impact is not absolute and may vary to some extent. Therefore, ongoing and careful attention to the interaction of prompt quality and model performance remains crucial.

\begin{table}[!htbp]
        \centering
        \scriptsize
        \caption{The Improvement of Average Score after Prompt Clarification}
        \label{tab:rewrittenPrompt}
        \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
       \textbf{Dataset} &Wk-type&\textbf{CodeT5} & \textbf{UnixCoder} &\textbf{CodeRL} &\textbf{CodeGen} & \textbf{ChatGPT}\\ \hline
      \multirow{5}{*}{CoNaLa} &I.i &0.07	&0.12	&0.07 &0.10 &0.03 \\ \cline{2-7}
&I.ii& 0.01 &0.07 &-0.01 &0.14 &0.01 \\ \cline{2-7}
&I.iii & 0.01 &	0.07 &-0.02	&0.14 &0.003 \\ \cline{2-7}
&II & 0.06& 0.04 &0.03 &0.05 &0.05 \\ \cline{2-7}
&III & 0.08	&0.06 &0.07 &0.02 &0.02 \\ \hline

       \multirow{2}{*}{HumanEval}&I.i &-0.16 &0.09 &0.17&0.10 &0.09 \\ \cline{2-7}
       &II &-0.04 &0.09 &0.16 &-0.02 &0.01 \\ \hline
       DS-1000 &II & 0.03 & -0.06 &0 &0.02 &0 \\ \hline
        \end{tabular}
\end{table}



% \noindent \textbf{H2: Better readability of prompts, better quality of the generated code.} Previous studies have demonstrated that the quality of prompts can affect the performance of large models on tasks such as program repair \cite{cao2023study}, vision-based generation \cite{jin2022good} and code search \cite{10.1145/3236024.3236065} to a certain extent. However, these studies did not reveal what constitutes a good prompt for PLMs. We propose an initial guess that good readability might be an essential feature of a high-quality prompt, since high readability often requires clarity and specificity, and avoids vagueness. Thus, we put forth hypothesis H0: better readability of prompts leads to better quality of the generated source code. 

% To test this hypothesis, we need to measure the prompt readability firstly. Basically, the prompts in CoNaLa are consisted of pure natural language sequence. However, in some dataset, like HumanEval, the prompts may contain three parts: natural language (NL) intent description, contextual source code, and input-output examples. For better illustration, we show one example here. 

%  \begin{lstlisting}[breaklines, columns = flexible, basicstyle=\footnotesize, showstringspaces=false ]
%    def fix_spaces(text):
%     " " "
%     Given a string text, replace all spaces in it with underscores,
%     and if a string has more than 2 consecutive spaces, then replace
%     all consecutive spaces with - 
%     fix_spaces(``Example") == "Example"
%     fix_spaces(``Example 1") == "Example_1"
%     fix_spaces(`` Example 2") == "_Example_2"
%     fix_spaces(`` Example   3") == "_Example_3"
%     " " "
%  \end{lstlisting}
 
%     Considering that source code is generally more formal than NL sequences, there should be different ways to evaluating their readability. Besides, examples are also represented formally and easily, often improving the readability of prompts. Thus, we define the readability level of prompts $RA_{prompt}$ as the sum of 
%     the readability level of the  code part  $RA_{code}$ and the NL sequence $RA_{nl}$. Besides, due to the clarification function of examples, we minus an adjustment factor. 
    
%     The readability of source code $RA_{code}$ is defined as the sum of keywords, operators, assignment operations, and the bracket depth, because these elements indicate the complexity of source code. And we employ \emph{Flesch-Kincaid Grade Level}, a widely-used metric to show what educational level a person will need in order to understand a particular text, to measure the readability of NL part. For the example part, we use $len_{example}/len_{nl}$, because generally, (more) longer examples provide better clarification. Parameters of $\alpha, \beta, \gamma$ adjust the weights of these three parts. And $\alpha$ and $\beta$ use the proportion of code and NL description in the whole prompt, respectively. $\gamma$ is designed to balance the example ratio (i.e., $\frac{len_{example}}{len_{nl}}$) with the NL intent readability. We use 20 because statistical analysis shows that $RA_{nl}$ is about 20 times of the example ratio.
    
%         \begin{equation}
%         \small
%         \setlength{\abovedisplayskip}{0pt}
%         \setlength{\belowdisplayskip}{0pt}
%             \begin{aligned}
%                  RA_{prompt}= \alpha * RA_{code} +\beta * RA_{nl} - \gamma* \frac{len_{example}}{len_{nl}} \\
%                  RA_{code} = N_{keyword} + N_{operator}+ N_{assignment} + N_{bracket\_depth} \nonumber
%             \end{aligned}
%             %\label{eq_s}
%         \end{equation}

%         %  \begin{equation}
%         %  \small
%         %  \begin{aligned}
%         %     RA_{code} = N_{keyword} + N_{operator}+ N_{assignment} + N_{bracket\_depth} 
%         %     \end{aligned}
%         %     \label{equ:ra_code}
%         % \end{equation}
%         \vspace{1.5em}
%         Based on the aforementioned definitions, we investigate whether $RA_{prompt}$ is correlated with the quality of the generated code for different models. For each dataset-model combination, we calculate the correlation coefficient between $RA_{prompt}$ and CodeBLEU of the generated code using Pearson's measure at a 0.05 significance level. We choose CodeBLEU as it is a comprehensive metric that considers not only basic sequence matching (as in Bleu-4) but also syntactic and code semantic matching. Table \ref{tab:correlation} displays the results, where `r' represents correlation and `p' indicates significance.
        
%         %Correlation score is a measure ranging from -1 to +1, indicating the degree of association between two sets of data. Significance is an estimation of the probability of the correlation being due to random chance. A significance of 0 indicates a high confidence in the correlation, while a high value indicates a high chance for independence between the variables. We use Pearson's measure and 0.05 of significance level. Table \ref{tab:correlation} shows the results, where r, p mean correlation and significance respectively.

%         \begin{table}[htbp]
%         \centering
%         \footnotesize
%         \caption{Correlations between prompt readability and CodeBleu.}
%         \label{tab:correlation}
%         \begin{tabular}{|c|c|c|c|c|c|c|}
%         \hline
%         \multirow{2}{*}{\textbf{Models}} & \multicolumn{2}{c|}{\textbf{CoNaLa}} & \multicolumn{2}{c|}{\textbf{HumanEval}} & \multicolumn{2}{c|}{\textbf{DS-1000}} \\
%         \cline{2-7}
%         & \textbf{r} & \textbf{p} & \textbf{r} & \textbf{p} & \textbf{r} & \textbf{p} \\
%         \hline
%         \textbf{CodeT5} & \textbf{-0.102} & \textbf{0.022} & -0.041 & 0.604 & \textbf{-0.064} & \textbf{0.042} \\
%         \hline
%         \textbf{UnixCoder} & \textbf{-0.139} & \textbf{0.002} & -0.131 & 0.093 & 0.026 & 0.412 \\ 
%         \hline
%         \textbf{CodeRL} & \textbf{-0.100} & \textbf{0.025} &\textbf{ -0.157} &\textbf{ 0.044} & \textbf{-0.067} & \textbf{0.034} \\
%         \hline
%         \textbf{CodeGen} & \textbf{-0.120} &\textbf{0.007} & \textbf{-0.265} & \textbf{0.001} & \textbf{-0.129} & \textbf{0} \\
%         \hline
%         \end{tabular}
%         \end{table}

%         We observe that for CoNaLa, there is a significant negative correlation between prompt readability and the quality of generated code for all four models. Similar results can be seen for HumanEval and DS-1000 with the two larger models CodeGen and CodeRL, in which we do not perform fine-tuning on these two datasets. However, for CodeT5 and UnixCoder with fine-tuning, this phenomenon is relatively less significant.
        
%         Note that CoNaLa prompts consist of pure NL intent descriptions, without illustrative examples or source code. This suggests that better readability of NL prompts tends to result in higher-quality generated code. This rule also applies when using off-the-shelf pre-trained models, but the negative correlation is only marginal for the model with fine-tuning in the dataset. Anyway, improving the readability of prompts should be an effective way of enhancing the PLMs' performance.

%         In practice, models evolve continuously. We would like to know whether the improved prompts work better on different models too. Thus, we evaluate the second hypothesis.
     
%      \vspace{0.5em}
     
   % \noindent \textbf{H2: Different models achieve high agreement on the quality of prompts.} In other words, if model $\alpha$ can generate a better code for a specific prompt $p$, it is very likely that model $\beta$ can produce higher quality code too, compared to other prompts. If this hypothesis is true, the quality of prompts is transferable across different models, indicating the practical significance of improving prompts.

   %  We expect to evaluate the agreement between the qualities of code generated by the four models for each prompt in the three datasets. Here we employ Intraclass Correlation Coefficient (ICC) \cite{icc} to assess the agreement, and use \emph{CodeBLEU} as the quality metric. ICC is a statistical measure used to assess the degree of similarity among observations within groups. CodeBLEU is selected due to the same reason in the H1 evaluation. Considering that CodeT5 and UnixCoder have been fine-tuned on HumanEval and DS-1000, and different operations may effect the consistency, we evaluate the agreement of the four models on CoNaLa, two smaller models on HumanEval and DS-1000, and the two bigger models on these two datasets. Table \ref{tab:consistency} shows the ICC results.
    

   %   \begin{table}[!htbp]
   %  \caption{Consistency of models on the three datasets.}
   %  \label{tab:consistency}
   %  \centering
   %  \footnotesize
   %  \begin{tabular}{|p{0.8cm}|p{1.0cm}|p{0.8cm}|p{0.8cm}|p{0.9cm}|p{0.9cm}|p{0.6cm}|}
   %  \hline
   %  \multirow{2}{*}{\textbf{Metric}} & \multirow{2}{*}{\textbf{CoNaLa}}& \multicolumn{2}{c|}{\textbf{HumanEval}} & \multicolumn{2}{c|}{\textbf{DS-1000}}& \multirow{2}{*}{\textbf{AVG}}\\ \cline{3-6} 
   %  & & T5\&UC & CR\&CG & T5\&UC & CR\&CG & \\ \hline
   %  \textbf{ICC} & 0.903 & 0.86 &0.46 &0.81  & 0.53 & 0.74 \\ \hline
   %  \multicolumn{7}{l}{T5:CodeT5, UC:UnixCoder, CR:CodeRL, CG:CodeGen} \\
   % % \textbf{B.-A.} & 0.05 & 0.09 &  0.06 & 0.07 \\ \hline
   %  \end{tabular}
   %  \end{table}

   %  We can see that on average, nearly good agreement has been achieved on the three datasets ($ 0.90 > ICC \ge 0.75 $: good reliability \cite{icc}). Especially, excellent reliability has been achieved on CoNaLa ($ICC\ge 0.90$). Besides, good reliability has been achieved by the two smaller models on both HumanEval and DS-1000. However, the two bigger models have poor agreement on these two datasets. This implies that pre-trained models with consistent operations (e.g., fine-tuning) achieve good agreement on the quality of prompts.
    
   % \vspace{0.5em}
   
   % \noindent \textbf{H3: Third-party libraries usage is still a weak link for the automated code generation task.}    In order to investigate whether the model's performance is significantly worse when the prompt involves third-party libraries, we perform Mann-Whitney U test \cite{mann1947test}. First, we calculated the comprehensive performance scores by reusing the measure in Section \ref{subsec:zone} (i.e., $\emph{score}=(CodeBLEU + EditSim)/2$) for the prompts involving third-party libraries and those not involving them. Subsequently, we conducted a Mann-Whitney U test to compare the scores of these two sets. Table \ref{tab:third-party} shows the average scores on the three datasets and the p-value of U test with the significance level of 0.05.
    
   %  \begin{table}[!htbp]
   %  \caption{Mann-Whitney U test of Third-party libraries-based code generation.}
   %  \label{tab:third-party}
   %  \centering
   %  \footnotesize
   %  \begin{tabular}{|c|c|c|c|}
   %  \hline
   %  \textbf{Models} &\textbf{Library Scores}&\textbf{Non-library Scores}&\textbf{P}\\ \hline
   %  \textbf{CodeRL} & 35.15 & 42.52& \textbf{0.010 }\\ \hline
   %  \textbf{CodeGen} & 36.89 &42.50&\textbf{0.033}\\ \hline
   %  \textbf{CodeT5} & 36.28 & 40.33 &0.197 \\ \hline
   %  \textbf{Unixcoder} & 33.01 & 40.86 & \textbf{0.004} \\ \hline
   %  \end{tabular}
   %  \end{table}

   %  From Table \ref{tab:third-party}, it is evident that for the all four models, the scores of the pairs without third-party-library involving achieve approximately 20\% gains than those involving third-party libraries. Additionally, the results of the Mann-Whitney U test indicate that these differences are statistically significant among the three models. We suggest that the PLMs developers/researchers should pay more attention on this topic.



    
    %Since these zones are the result of intersections from four models, this may indicate the universality of single answer biases in benchmark, reflecting the importance of diverse answers. Additionally, the weakness of complex prompt is emphasized in both HumanEval and DS-1000, where prompts are longer, as shown in Table \ref{tab:dataset}. 

    \noindent \textbf{RQ2: Weakness applicability for ChatGPT.}

Our study seeks to ascertain if the six categories of prompt- and model-related weaknesses identified in medium-scale code-PLMs also apply to  ChatGPT. In particular, our objectives are: 1) to evaluate ChatGPT's efficacy in dealing with prompt-related weaknesses (Types I-III as detailed in Section 4.1), and 2) to assess its capacity to overcome inherent model-related weaknesses (Types IV-VI). We have excluded single-answer biases from this evaluation since they do not represent fundamental issues with the models themselves.

For prompt-related weaknesses, we used the samples in RQ1 directly (Table \ref{tab:randomSample}). For model-specific weaknesses, we randomly selected 30 instances showcasing each type of weakness from each of the three datasets. Hence, the selected data could span any grade level. If the total number of samples was less than 30, all available examples were used — for instance, there were only 9 entries that displayed incorrect API usage in the HumanEval dataset. The threshold of 30 was chosen because there are more instances of model-related weaknesses than prompt-related ones.
%As part of our examination of prompt-related weaknesses, we referred directly to the examples provided in Table 4. For model-specific weaknesses, we randomly selected 30 instances showcasing each type of weakness from each of the three datasets. Hence, the selected data could span any grade level. If the total number of samples was less than 30, all available examples were used — for instance, there were only 9 entries that displayed incorrect API usage in the HumanEval dataset.

Given that problem types vary across different datasets, we opted for distinct questioning prompts for each. For CoNaLa, ChatGPT was tasked with generating code snippets for given prompts, while for HumanEval and DS-1000, it was prompted to provide code completions in the given context. All prompts were designed as single-turn conversations, utilizing the GPT-3.5-Turbo model. The quality of the produced code was then gauged through metrics outlined in Section \ref{subsec:rep}, with results presented in Table \ref{tab:chatgpt}. We also included the ratio of samples successfully passing the given test cases in HumanEval and DS-1000, in the last column.

ChatGPT exhibits all kinds of weaknesses under scrutiny. For prompt-related weaknesses, it shows greater tolerance towards \emph{inconsistency} (Type I.iii), complex texts (Type II) and grammar errors (Type III), but fares poorly with incomplete prompts (Type I.ii). As for model-related weaknesses, performance was generally satisfactory, with automatic evaluations passed at rates of 22/60, 14/39, and 6/23 respectively. For instance, ChatGPT demonstrated the awareness of knowledge of IP address upper limits being 255 and comprehended rules for crafting regular expressions.

When compared to our chosen set of medium-scale code-PLMs, ChatGPT exhibited notable enhancements in the selected cases. For example, ChatGPT achieved a CodeBLEU score of 29.72, surpassing CodeRL's score of 23.44 and CodeGen's 21.68. It also significantly improved the number of successful responses, 50 out of 145 data samples with test cases (2 for CodeGen, and 1 for CodeRL). Worth noting, however, is ChatGPT’s declining performance on EditSim and Exact Match metrics. This could be attributed to ChatGPT's propensity to produce comprehensive code, which includes defining variables not specified in the prompt. As a result, the longer generated code could be behind the decline in these two metrics.

% When compared to our chosen set of medium-scale PLMs, ChatGPT exhibited notable enhancements in these challenging scenarios. For example, ChatGPT achieved a CodeBLEU score of 29.72, surpassing CodeRL's score of 23.44 and CodeGen's 21.68. ChatGPT also significantly improved the number of successful responses, with correct answers provided for 50 out of 145 data samples. Worth noting, however, is ChatGPT’s declining performance on EditSim and Exact Match metrics. This could be attributed to ChatGPT's propensity to produce comprehensive code, which includes defining variables not specified in the prompt. As a result, the longer generated code could be behind the decline in these two metrics.

% Our investigation aims to determine whether the six types of prompt- and model-related weaknesses identified in medium-scale pre-trained models are applicable to state-of-the-art commercial large language models like ChatGPT. Specifically, we want to examine: 1) if ChatGPT can effectively handle prompt-related weaknesses (Types I-III as described in Section \ref{subsec:promptWeakness}), and 2) if it can surmount the model inherent weaknesses (Types IV-VI). The evaluation does not include single-answer biases, as they are not fundamentally issues with the models themselves.

% For prompt-related weaknesses, we directly employed the examples provided in Table \ref{tab:randomSample}. As for model-specific weaknesses, we randomly selected 30 entries exhibiting each type of weakness from each of the three datasets. Consequently, the sampled data could be distributed across any grade. In cases where the total number of samples was below 30, we utilized all available examples (e.g., there were only 9 entries demonstrating incorrect API usage in the HumanEval dataset).

% The problem types vary across different datasets, so we utilized different questioning prompts. For the Conala dataset, ChatGPT was prompted to provide code snippets, while for HumanEval and DS-1000, it was prompted for code completions in the given context. All prompts were designed as single-turn conversations, utilizing the GPT-3.5-Turbo model. Subsequently, the quality of generated code was evaluated through metrics in Section \ref{subsec:rep}, and the results are shown in Table \ref{tab:chatgpt}. For HumanEval and DS-1000, we also list the ratio of samples passing the given test cases.

\begin{table}[!htbp]
\centering
\caption{Performance of ChatGPT on Various Weaknesses}
%\scriptsize
\footnotesize
\label{tab:chatgpt}
\begin{tabular}{|p{1.4cm}|p{0.2cm}|p{0.5cm}|p{0.5cm}|p{0.75cm}|p{1.0cm}|p{0.7cm}|}
\hline
\multicolumn{2}{|c|}{Category} & Num & EM & EditSim & CodeBLEU & pass@1 \\ \hline
\multirow{6}{1.5cm}{\centering Prompt-related\\Weakness}
& I & 36 & 0.00 & 17.89 & 30.47 & 1/1 \\ 
& I.i & 16 & 0.00 & 18.14  & 29.59 & 1/1 \\ 
& I.ii & 15 & 0.00 & 16.58 & 24.32 & - \\ 
& I.iii & 15 & 0.00 & 19.33  & 31.13 & - \\ 
& II & 37 & 0.00 & 29.10 & 31.55 & 7/22 \\ 
& III & 5 & 0.00 & 18.32 & 32.67 &- \\ \hline
\multirow{3}{1.5cm}{\centering Model-related\\Weakness}
& IV & 90 & 3.33 & 33.02 & 28.21 & 22/60 \\ 
& V & 69 & 1.45 & 30.39 & 31.38 & 14/39 \\ 
& VI & 38 & 0.00 & 30.51 & 27.47 & 6/23 \\ \hline
\end{tabular}
\end{table}

%Generally speaking, all kinds of weakness exist in ChatGPT. For prompt-related weaknesses, ChatGPT exhibited better tolerance towards grammar errors (type I.iii) and complex text (type I), but worst tolerance towards incompleteness (Type I.ii). For model-related weaknesses, it performed relatively well overall, passing 22/60, 14/39, and 6/23 automatic evaluations (pass@1) respectively, suggesting the potential for improvements in these aspects with stronger models. For example, in terms of domain knowledge, ChatGPT demonstrated awareness of the upper limit of IP addresses being 255 and understanding the rules for writing regular expressions.% However, over 65\% of the problems still remained unresolved, indicating that model-related weaknesses persist in ChatGPT.  %In the all 270 samples, it could not overcome over 65\% of the identified weaknesses (passing only 34.48\% of the examples), with the highest CodeBLEU being only 32.67.

%ChatGPT demonstrated a moderate capability in handling prompt-related weaknesses with a CodeBLEU of 31.56. 
%For prompt-related weaknesses, ChatGPT exhibited better tolerance towards grammar errors (type I.iii) and complex text (type II), but worst tolerance towards incompleteness was the lowest (Type I.ii). For model-related weaknesses, it presents better tolerance with the API usage weakness observed in medium-model PLMs. %This indicates that as a general large-scale model, ChatGPT can relatively accurately handle complex text and grammar errors but struggles with incomplete descriptions.

%Meanwhile, for model-related weaknesses (types IV-VI), ChatGPT performed relatively well overall, passing 22/60, 14/39, and 6/23 automatic evaluations (pass@1) respectively, suggesting the potential for improvements in these aspects with stronger models. For example, in terms of domain knowledge, ChatGPT demonstrated awareness of the upper limit of IP addresses being 255 and understanding the rules for writing regular expressions. However, over 65\% of the problems still remained unresolved, indicating that model-related weaknesses persist in ChatGPT.

% Compared to our selected medium scale PLMs, ChatGPT achieved improvements in these problematic cases. For example, ChatGPT obtained 29.72 CodeBLEU, outperforming CodeRL with 23.44 and CodeGen with 21.68. Additionally, ChatGPT demonstrated significant improvement in the number of passed questions (50 out of 145 data samples). %These results suggest that ChatGPT indeed outperforms the selected specialized code generation models in code generation ability. 
% MeanWhile, it's worth noting that ChatGPT's performance on EditSim and Exact Match metrics declined. This maybe attributed to ChatGPT's tendency to provide complete code, including defining variables not specified in the prompt, resulting in longer generated code and causing the decline in these two metrics.

% Despite ChatGPT's impressive performance in code generation, we still observed weaknesses within ChatGPT. It could not overcome over 65\% of the identified weaknesses (passing only 34.48\% of the examples), with the highest CodeBLEU being only 32.67.

% For Prompt-Related Weaknesses, ChatGPT demonstrated a moderate capability in handling prompt-related weaknesses with a CodeBLEU of 31.56. It exhibited good tolerance towards grammar errors and complex text (32.67 and 31.55, CodeBLEU respectively), but its tolerance towards incompleteness was the lowest (CodeBLEU only at 24.32). This indicates that as a general large-scale model, ChatGPT can relatively accurately handle complex text and grammar errors but struggles with incomplete descriptions.

% Regarding Model-Related Weaknesses, ChatGPT showed a certain level of capability in overcoming inherent model-related weaknesses (CodeBLEU of 29.02, passing 42 automatic evaluations). For types IV-VI, ChatGPT performed relatively well overall, passing 22, 14, and 6 automatic evaluations respectively, suggesting the potential for improvements in these aspects with stronger models. For example, in terms of domain knowledge, ChatGPT demonstrated awareness of the upper limit of IP addresses being 255 and understanding the rules for writing regular expressions. However, over 65\% of the problems still remained unresolved, indicating that model-related weaknesses persist in ChatGPT.

%test
\setParDefTest
